Fairness Behind a Veil of Ignorance: A Welfare Analysis for Automated Decision Making

We draw attention to an important, yet largely overlooked aspect of evaluating fairness for automated decision making systems---namely risk and welfare considerations. Our proposed family of measures corresponds to the long-established formulations of cardinal social welfare in economics, and is justified by the Rawlsian conception of fairness behind a veil of ignorance. The convex formulation of our welfare-based measures of fairness allows us to integrate them as a constraint into any convex loss minimization pipeline. Our empirical analysis reveals interesting trade-offs between our proposal and (a) prediction accuracy, (b) group discrimination, and (c) Dwork et al.'s notion of individual fairness. Furthermore and perhaps most importantly, our work provides both heuristic justification and empirical evidence suggesting that a lower-bound on our measures often leads to bounded inequality in algorithmic outcomes; hence presenting the first computationally feasible mechanism for bounding individual-level inequality.

==> analysis.tex <==
\section{Analysis}\label{sec:analysis}

Uniform convergence in the sense of~\citep{balcan2018envy}?

%Our tech- nical focus is the generalizability of envy-free classification, i.e., understanding whether a classi- fier that is envy free on a sample would be almost envy free with respect to the underlying distribu- tion with high probability.

==> intro_old.tex <==
\section{Introduction}
% Background
Algorithmic decision making systems are increasingly employed in a wide range of socially consequential domains---examples include employment~\citep{hiring}, credit lending~\citep{whitecase}, policing~\citep{policing}, and criminal justice~\citep{sentencing}. Decisions made in this fashion directly impact people's lives and may potentially affect certain individuals or social groups negatively~\citep{sweeney2013discrimination,propublica,guardian_beauty}. This has recently led to an active area of research into quantifying and guaranteeing fairness for machine learning~\citep{dwork2012fairness,kleinberg2016inherent,hardt2016equality}. 
Much of the existing work has been devoted to the study of algorithmic \emph{discrimination} (also called \emph{statistical}- or \emph{group}-level fairness by the machine learning community), whereas only a handful of studies have addressed algorithmic \emph{fairness} (also known as \emph{individual}-level fairness). 
% Related work
\citet{dwork2012fairness} first formalized the notion of individual fairness for classification learning tasks, requiring that two individuals who are similar with respect to the task at hand receive similar classification outcomes. More recently, \citet{speicher2018a} proposed a new measure for quantifying individual unfairness, utilizing income inequality indices from economics and applying them to \emph{algorithmic benefit} distributions. Both of these formulations focus solely on the \emph{inter-personal} comparison of algorithmic outcomes across individuals and do not account for \emph{risk} and \emph{welfare} considerations (as illustrated in Example~\ref{ex:compar}). Moreover, there do not exist efficient, exact mechanisms for bounding either of these formulations.

% Our proposal
In this paper, we propose a natural family of measures for evaluating individual\footnote{While our main focus in this work is on individual-level fairness, our ideas are readily applicable to group-level fairness, as well.} fairness, corresponding to long-established notions of \emph{cardinal social welfare} in economics. Our proposal is motivated by the fundamental concept of \emph{veil of ignorance} in political philosophy~\citep{rawls2009theory}, and is operationalized utilizing models of risk attitude in economics~\citep{harsanyi1953cardinal,harsanyi1955cardinal}. 
In order to evaluate fairness behind a veil of ignorance, Rawls puts forward the following thought experiment (recast to reflect our setting of interest): imagine an agent who knows nothing about the particular individual they will be within the society/population, and is asked to select among a set of algorithmic alternatives (e.g. to choose whether their recidivism risk is going to be predicted using neural networks or decision trees~\citep{propublica}). In this hypothetical original/ex-ante position, if the agent is \emph{rational}, they would aim to minimize risk and insure against unlucky events in which they turn out to be an individual with low algorithmic benefit. This risk is precisely what our proposal seeks to quantify. Our core idea consists of computing the expected utility of a randomly chosen, \emph{risk-averse} individual as the result of being subject to algorithmic decision making. Our family of measures contains the Rawlsian max-min fairness as special case. 
%
The following example further illustrates the key difference between our proposal in contrast to~\citep{speicher2018a} and \citep{dwork2012fairness}. 
\begin{example}\label{ex:compar}
Consider two decision making models A, B each resulting in a different benefit distribution across 4 individuals $i=1,2,3,4$ all with ground truth label $1$ (we will precisely define in Section~\ref{sec:model} how individual benefits are computed, but for the time being, suppose benefits are equivalent to regression outcomes). Model A assigns the same benefit of 0.9 to every individual, whereas model B assign a benefit of 0.6 to individual 1, a benefit of 1 to individuals 2 and 3, and a benefit of 1.1 to individual 4. 
%
\begin{figure}[h!]
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{Figures/example.png}
  \label{fig:example}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
\begin{tabular}{| l | c | c | }
  \hline			
    Measure / model & A & B \\
    \hline
  social welfare ($\alpha=0.5$) & 0.9487 & \textbf{0.9559} \\
  gen. entropy ($\alpha=2$) & \textbf{0} & 0.0054 \\
  Dwork et al.'s conditions & \textbf{0} & 0.25 \\
  mean difference & \textbf{0} & 0.25 \\
  negative Residual diff. & \textbf{0} & 0.4 \\
  positive Residual diff. & \textbf{0} & 0.05 \\
  \hline  
\end{tabular}
\end{minipage}
\end{figure}

Both ~\citep{speicher2018a} and \citep{dwork2012fairness} notions of individual fairness deem model A fairer than B, as it results in perfect equality and treats all individuals similarly. Also note that neither of the two models Pareto-dominates the other (individual 1 prefers model A, whereas individuals 2,3,4 prefer model B). In contrast, assuming individuals are not acutely risk-averse ($\alpha > 0.5$, where $\alpha$ is the risk aversion parameter---to be defined in Section~\ref{sec:model}) our approach considers B a fairer alternative.
\end{example} 

The convex formulation of our measures allows us to integrate them as a constraint into any convex loss minimization pipeline, and solve the resulting problem efficiently and exactly. Our empirical analysis reveals interesting trade-offs between our proposal and (a) prediction accuracy, (b) group discrimination, (c) \citeauthor{dwork2012fairness}'s notion of individual fairness. Furthermore and perhaps most importantly, our work presents both theoretical and empirical evidence suggesting that putting a constraint on social welfare leads to bounded algorithmic inequality---as recently proposed by~\citep{speicher2018a}---hence presenting the first computationally feasible mechanism for bounding individual-level fairness.

==> mechanism.tex <==
\section{Fairness Mechanisms}

%Having established the existence of trade-offs between our measure and that of \citet{dwork2012fairness}, in this section we present a heuristic for simultaneously bounding welfare and Dwork et al.'s notion of individual fairness. 
In this section we propose heuristic mechanisms for bounding individual fairness of \cite{dwork2012fairness} and \cite{speicher2018a}.

The first heuristic we propose works as follows: it first solves the unconstrained ERM. Next it finds the pairwise constraints that are violated by a margin of at least $\delta$. Finally, it adds these constraints to ERM and solve the resulting optimization. Figure~\ref{fig:dwork} shows the performance of this heuristic as $\delta$ varies.

\iffalse
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/avg_viol.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/num_viol.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/num_viol_delta.png}
    \end{subfigure}
%        \begin{subfigure}[b]{0.32\textwidth}
%        \includegraphics[width=\textwidth]{Figures/num_const.png}
%    \end{subfigure}
%        \begin{subfigure}[b]{0.32\textwidth}
%        \includegraphics[width=\textwidth]{Figures/calc_time.png}
%    \end{subfigure}
    \caption{Illustration of the heuristic for Dwork et al.}\label{fig:dwork}
\end{figure*}
\fi

The second mechanism we propose works as follows: it first finds a compressed representation of the training data (e.g. an epsilon-net); then solves ERM subject to pairwise constraints among members of the compressed representation.

The mechanism we propose for Speicher et al. works as follows: Suppose the mean utility is fixed and is equal to $\mu$. Solve the following optimization:
\begin{eqnarray*}
\min_{\vtheta \in \reals^k} && \sum_{i = 1}^n (\vtheta.\vx_i - y_i)^2 \\
 \text{s.t.} && \sum_{i=1}^n \left(\frac{\vtheta.\vx_i - y_i + 1}{\mu}\right)^2-1 \geq 2n\tau \\
 && \sum_{i=1}^n (\vtheta.\vx_i - y_i + 1) = n\mu
\end{eqnarray*}
Note that the above is a convex function of $\vtheta$ and therefore can be solved accurately. Solve the above optimization for different values of $\mu$ and pick the one that minimizes loss. 
